SmartChunk Retrieval: Query-Aware Chunk Compression with Planning for Efficient Document RAG

Retrieval-augmented generation (RAG) has strong potential for producing accurate and factual outputs by combining language models (LMs) with evidence retrieved from large text corpora. However, current pipelines are limited by static chunking and flat retrieval: documents are split into short, predetermined, fixed-size chunks, embeddings are retrieved uniformly, and generation relies on whatever chunks are returned. This design brings challenges, as retrieval quality is highly sensitive to chunk size, often introduces noise from irrelevant or misleading chunks, and scales poorly to large corpora. We present SmartChunk retrieval, a query-adaptive framework for efficient and robust long-document question answering (QA). SmartChunk uses (i) a planner that predicts the optimal chunk abstraction level for each query, and (ii) a lightweight compression module that produces high-level chunk embeddings without repeated summarization. By adapting retrieval granularity on the fly, SmartChunk balances accuracy with efficiency and avoids the drawbacks of fixed strategies. Notably, our planner can reason about chunk abstractions through a novel reinforcement learning scheme, STITCH, which boosts accuracy and generalization. To reflect real-world applications, where users face diverse document types and query styles, we evaluate SmartChunk on five QA benchmarks plus one out-of-domain dataset. Across these evaluations, SmartChunk outperforms state-of-the-art RAG baselines, while reducing cost. Further analysis demonstrates strong scalability with larger corpora and consistent gains on out-of-domain datasets, highlighting its effectiveness as a general framework for adaptive retrieval.

==> app_backup.tex <==
\section{Appendix}
You may include other additional sections here.

\section{Why Different Chunk Size}

Short, contiguous spans rarely suffice for long-range reasoning. For example, a typical question in NarrativeQA \cite{kovcisky2018narrativeqa} is “What motivates the main character’s change of heart by the end?”. This is not answerable by extracting localized text. It requires integrating information spread widely across the entire text. While oversized chunks introduce a different problem: important fine-grained details are blurred or lost, making it harder to ground accurate answers. At the same time, embedding models have limited effective context and degrade on very long inputs, while LLMs remain inefficient at leveraging long context. Not all queries require long context in the first place. For example, in the QASPER dataset of questions about NLP research papers~\cite{dasigi2021dataset}, many answers are extractive and confined to a single paragraph. A question such as “What other political events are included in the database?” can typically be answered from a sentence- or paragraph-level chunk in the methods section, without needing the entire paper as context. Using overly large chunks for such questions can retrieve the relevant information with surrounding noise, hurting retrieval accuracy and answer quality.

\section{Experimental details} \label{app:exp_detail}
\input{iclr2026/ablation}
\section{Algo}
\input{iclr2026/alg}
% \begin{algorithm}
% \small
% \caption{STITCH:Solve with RL, Then Imitate To Close Holes}
% \begin{algorithmic}[1]
% \Require Dataset $\mathcal{D}$, current policy $\pi_\theta$, sampling number $G$, a list of keywords for splitting episodes $[w_0,w_2,...,w_J]$
% \Procedure{\texttt{STITCH}}{$\mathcal{D},\pi_\theta,G,[w_0,w_2,...,w_J]$}

%     \For{$\text{step}=1,2,...,N$}
%     \State Sample a batch $\mathcal{D}_b$ from $\mathcal{D}$
%     \State Update the old policy model $\pi_{\text{old}}\gets \pi_\theta$
%     \For{each question and expert solution pair $(Q,S)$ in $\mathcal{D}_b$}
%     \State $[R_1,R_2,...,R_G], \rho\gets$ \texttt{EAS}($Q,S,\pi_\theta,G,[w_0,w_2,...,w_J]$) \Comment{Episode Anchor Search (\texttt{EAS)}}
%     \State Add the $(Q,\rho),R_i$ to the buffer.
%     \EndFor
%     \State For each $(Q,\rho),o_i$ in the buffer, compute $\hat{A}_{i,t}$ for the $t$-th token of $o_i$ \Comment{\Cref{eq:adv}}
%     \EndFor
%     \For{$\text{iteration}=1,2,...,T$}
%     \State Update the policy model $\pi_\theta$ by maxmizing the STITCH objective \Comment{\Cref{eq:BREAD_obj}}
%     \EndFor
%     \State \textbf{return} $\pi_\theta$
% \EndProcedure
% \Procedure{\texttt{EAS}}{$Q,S,\pi,G,[w_0,w_2,...,w_J]$}
%     \State $[R_1,R_2,...,R_G] \gets \pi(Q)$ \Comment{Sample $I$ responses for question $Q$ with current policy $\pi$}
%     \State $p_{\text{correct}} \gets \mathtt{compute\_correct\_probability}([R_1,R_2,...,R_G],S)$ 
%     \State \Comment{compute correct probability based on responses and the gold solution}
%     \If{$0< p_{\text{correct}}$}
%         \State \textbf{return} $[R_1,R_2,...,R_G], NA$
%     % \ElsIf{another condition}
%     %     \State ...  % do something else
%     \Else
%         \State $[e_0,e_1,...,e_K] \gets\mathtt{split\_episodes}(S,[w_0,w_2,...,w_J])$
%         \State \textbf{return} $\mathtt{BINARY\_SEARCH\_AND\_GENERATE}(Q,S,\pi,G,[e_1,e_2,...,e_K],0,K)$ 
%         % \State \Comment{\textcolor{red}{Maybe some edge cases missing here. Maybe need fix}}
%     \EndIf
%     % \While{$b \ne 0$}
%     %     \State $r \gets a \bmod b$
%     %     \State $a \gets b$
%     %     \State $b \gets r$
%     % \EndWhile
%     % \State \textbf{return} $a$
% \EndProcedure
% % \Procedure{\texttt{binary\_search\_and\_generate}}{$Q,S,\pi,I,[e_1,e_2,...,e_K],L,R$}
% %     \State $[e_1,e_2,...,e_K] \gets\mathtt{split\_episodes}(S,[w_0,w_2,...,w_J])$
% %     \State $M=\frac{L+R}{2}$
% %     \State $[R_1,R_2,...,R_I] \gets \pi([Q,e_0,e_1,...,e_M])$
% %     \State $p_{\text{correct}} \gets \mathtt{compute\_correct\_probability}([R_1,R_2,...,R_I],S)$
% %     \If{$0 < p_{\text{correct}} < 1$}
% %         \State \textbf{return} $[R_1,R_2,...,R_I], S_{1:M}$
% %     \ElsIf{$p_{\text{correct}}=0$}
% %         \State $L=M,R=R,M=\frac{L+R}{2}$
% %         \State \textbf{return} $\mathtt{binary\_search\_and\_generate}(Q,S,\pi,I,[e_1,e_2,...,e_K],L,R)$
% %     \Else
% %         \State $L=L,R=M,M=\frac{L+R}{2}$
% %         \State \textbf{return} $\mathtt{binary\_search\_and\_generate}(Q,S,\pi,I,[e_1,e_2,...,e_K],L,R)$
% %     \EndIf
% % \EndProcedure
% \end{algorithmic}
% \label{alg:STITCH}
% \end{algorithm}

% \begin{algorithm}[t]
% \caption{Data collection}
% \label{alg:data}
% \begin{algorithmic}[1]
% \Require Dataset $\mathcal{D} = \{(q, d)\}$ of queries $q$ and documents $d$
% \Ensure Planner $\pi_\theta$ that predicts chunk sizes
% \State Initialize planner $\pi_\theta$ and retriever $\mathcal{R}$
% \For{each $(q, d) \in \mathcal{D}$}
%     \State Build multi-level chunk tree for $d$
%     \State Retrieve top-$k$ chunks with $\mathcal{R}$
%     \State Generate answer with generator $\mathcal{G}$
%     \If{answer is correct}
%         \State Record $(\text{smallest\_chunk}, \text{largest\_chunk})$ as pseudo-label
%     \Else
%         \State Expand retrieval and retry until solved or unsolved
%     \EndIf
% \EndFor
% \State \textbf{SFT stage:} Train $\pi_\theta$ on pseudo-labels
% \State \textbf{RL stage:} Fine-tune $\pi_\theta$ with reward
% \[
%     r = \text{QA\_acc} - \alpha \cdot \text{latency} - \beta \cdot \#\text{chunks}
% \]
% \State \textbf{Distillation:} Use RL-refined planner outputs as anchors
% \State Generate diverse reasoning traces with multiple models
% \State Train final $\pi_\theta$ on stitched traces
% \State \Return planner $\pi_\theta$
% \end{algorithmic}
% \end{algorithm}
\section{Additional results} \label{app:exp}

==> eval.tex <==
\subsection{Evaluation}
\textbf{Graph Construction}
Time efficiency, Token Cost, 
\textbf{Retrieval}
Indexing efficiency, Retrieval efficiency
\textbf{Generation Accuracy}
Answer Accuracy
\textbf{Rationale Accuracy}

We consider different types of costs in this work \xz{here or in exp?}


==> formulation_backup.tex <==
\xz{shorten this part} We propose the \alg framework, depicted in \Cref{fig:framework}. When a new question $q \in \mathcal{Q}$ comes, and there is a reference corpus of documents $D$, which is segmented into a set of chunks $C$, the planner $\mathcal{P}$ predicts the smallest and largest chunk sizes to consider, using both document metadata and the query. In parallel, the Chunk Compression Encoder $\mathcal{E}$ builds a multi-level hierarchy by clustering smaller chunks and aggregating them into higher-level chunks. A high-level chunk embedding contains representation of the text summary of that cluster. The Chunk Compression Encoder $\mathcal{E}$ produces multi-level embeddings directly. Each high-level chunk thus encodes the semantics of a cluster without requiring explicit text summarization. This design eliminates repeated summary generation and enables efficient construction of multi-level embeddings for high-level chunks in the hierarchy. 

The retriever $\mathcal{R}$ and generator $\mathcal{G}$ follow the vanilla retrieval-augmented generation (RAG) system. The retriever’s objective is to identify a set of chunks such that the generator $\mathcal{G}$ can produce an accurate answer $a = \mathcal{G}(q, \mathcal{R}(q, C))$. Given the candidate set $C$, retrieval is performed by ranking chunks based on similarity between query embedding $e(q)\in \mathbb{R}^d$ and chunk embeddings $e(c)\in \mathbb{R}^d$. The top-$k$ chunks form:
$
\mathcal{R}(q, C) = \operatorname{TopK}\Big( \{ \langle e(q), e(c) \rangle : c \in C\} \Big),
$. This formulation is agnostic to the underlying retrieval method. Any advanced retriever can be incorporated in place of simple similarity search. Likewise, the generator $\mathcal{G}$ can be used with any model. In practice, large language models (e.g., GPT-family models) are typically used.

\textbf{Multi-level Chunking} We assume a multi-level chunk hierarchy $\mathcal{H}(D)$, where a document is represented at multiple granularities (e.g., sentence, paragraph, section, document or token spans such as 128, 256, 512, 1024 tokens) in a hierarchical structure. Higher-level chunks are constructed by aggregating lower-level ones through a summarizer $\mathcal{S}(\cdot)$. In practice, large language models (e.g., GPT) can serve as $\mathcal{S}$ to generate summarized text that forms a higher-level chunk. While raw fine-grained chunks preserve full semantic fidelity, they may fragment higher-level structure. Conversely, compressed chunks capture compact semantic summaries but may lose fine-grained details. This design enables the system to balance accuracy versus efficiency by adaptively mixing raw and compressed representations. \xz{didn't use $s$}
% \textbf{Multi-level Chunking} We assume a multi-level chunk hierarchy $\mathcal{H}(D)$, where a document is represented at multiple granularities (e.g., sentence, paragraph, section, document or token spans such as 128, 256, 512, 1024 tokens) in a hierarchical structure. Formally, let a document be denoted as $D = \{s_1, s_2, \dots, s_n\}$, where each $s_i$ is a minimal text unit (e.g., a sentence or a fixed-length segment of 125 tokens). Higher-level chunks are constructed by aggregating lower-level ones through a summarizer $\mathcal{S}(\cdot)$. In practice, large language models (e.g., GPT) can serve as $\mathcal{S}$ to generate summarized text that forms a higher-level chunk. For example, a paragraph-level chunk $c_5$ may be obtained by compressing four consecutive sentence-level chunks $c_5 = \mathcal{S}(c_1, c_2, \dots, c_4)$. While raw fine-grained chunks preserve full semantic fidelity, they may fragment higher-level structure. Conversely, compressed chunks capture compact semantic summaries but may lose fine-grained details. This design enables the system to balance accuracy versus efficiency by adaptively mixing raw and compressed representations. \xz{didn't use $s$}

\textbf{Planner} The planner, denoted by $\mathcal{P}$, is a model that predicts the appropriate chunking granularity for a given query. Formally, $\mathcal{P}(q,MetaData(D)) = \left(\text{level}_{\min}, \; \text{level}_{\max}\right)$, where $\text{level}_{\min}, \text{level}_{\max}$ denote the smallest and largest chunk levels sufficient to answer $q$ while minimizing overall cost (including multi-level chunk construction, retrieval, and generation), $MetaData(D)$ denote the metadata of documents. These predictions restrict the candidate retrieval set to: $C = \{ c \in \mathcal{H}(D) \;|\; \text{level}(c) \in [\text{level}_{\min}, \text{level}_{\max}] \}$.

\textbf{Chunk Compression Encoder}
Beyond text-level summarization, we introduce an embedding-level compression module, denoted as $\mathcal{E}(\cdot)$. Unlike $\mathcal{S}(\cdot)$, which produces summarized text chunks, $\mathcal{E}(\cdot)$ directly maps a set of fine-grained chunks into a single compressed embedding without generating intermediate text. Formally, given a group of lower-level chunks $\{c_1, c_2, \dots, c_4\}$ the module outputs : $e(c_5) = \mathcal{E}(c_1, c_2, \dots, c_4) \in \mathbb{R}^d$. where $e(c_5)$ represents a high-level semantic embedding that captures the aggregate meaning of the input chunks. In practice, $\mathcal{E}$ can be a pretrained embedding model such as SBERT encoder (multi-qa-mpnet-base-cos-v1)~\cite{reimers-gurevych-2019-sentence}, long-context embedding model (jina-embeddings-v3)~\cite{sturua2024jina} or a finetuned Chunk Compression Encoder.

==> method_backup.tex <==
\subsection{Overview of SmartChunk Retrieval}
\begin{figure}
\centering
% \vspace{-35pt}
\includegraphics[width=\textwidth]{img/smartchunk_iclr.pdf}
\vspace{-35pt}
\caption{\small{Overview of the \alg framework. Compared to vanilla RAG (bottom), which uses fixed chunking and flat retrieval, SmartChunk (top) introduces two key modules:  (1) a planner $\mathcal{P}$ that predicts the smallest and largest chunk sizes per query, enabling adaptive multi-level retrieval, and (2) a Chunk Compression Encoder $\mathcal{E}$ that produces compact, high-level embeddings for aggregated spans, lowering the cost of multi-level representation. These additions allow \alg to adapt chunking to query complexity and document structure, balancing accuracy and efficiency. Modules added by SmartChunk are shown in blue, while baseline modules from vanilla RAG are shown in black. The figure distinguishes between text (represented as blocks with horizontal lines) and embeddings (shown as solid-colored blocks).}}%\vspace{-15pt}
\label{fig:framework}
% \end{wrapfigure}
% \vspace{-15pt}
\end{figure}

We propose the \alg framework, depicted in \Cref{fig:framework}. When a new question $q \in \mathcal{Q}$ comes, and there is a reference corpus of documents $D$, which is segmented into a set of chunks $C$, the planner $\mathcal{P}$ predicts the smallest and largest chunk sizes to consider, using both document metadata and the query. In parallel, the Chunk Compression Encoder $\mathcal{E}$ builds a multi-level hierarchy by clustering smaller chunks (based on structure or context) and aggregating them into higher-level chunks. A high-level chunk embedding contains representation of the text summary of that cluster. The Chunk Compression Encoder $\mathcal{E}$ produces multi-level embeddings directly. Each high-level chunk thus encodes the semantics of a cluster without requiring explicit text summarization. This design eliminates repeated summary generation and enables efficient construction of multi-level embeddings for high-level chunks in the hierarchy. 

The retriever $\mathcal{R}$ and generator $\mathcal{G}$ follow the vanilla retrieval-augmented generation (RAG) system. The retriever’s objective is to identify a set of chunks such that the generator $\mathcal{G}$ can produce an accurate answer $a = \mathcal{G}(q, \mathcal{R}(q, C))$. Given the candidate set $C$, retrieval is performed by ranking chunks based on similarity between query embedding $e(q)\in \mathbb{R}^d$ and chunk embeddings $e(c)\in \mathbb{R}^d$. The top-$k$ chunks form:
$
\mathcal{R}(q, C) = \operatorname{TopK}\Big( \{ \langle e(q), e(c) \rangle : c \in C\} \Big),
$. This formulation is agnostic to the underlying retrieval method. Any advanced retriever can be incorporated in place of simple similarity search. Likewise, the generator $\mathcal{G}$ can be used with any model. In practice, large language models (e.g., GPT-family models) are typically used.


\textbf{Multi-level Chunking} We assume a multi-level chunk hierarchy $\mathcal{H}(D)$, where a document is represented at multiple granularities (e.g., sentence, paragraph, section, document or token spans such as 128, 256, 512, 1024 tokens) in a hierarchical structure. Formally, let a document be denoted as $D = \{s_1, s_2, \dots, s_n\}$, where each $s_i$ is a minimal text unit (e.g., a sentence or a fixed-length segment of 125 tokens). Higher-level chunks are constructed by aggregating lower-level ones through a summarizer $\mathcal{S}(\cdot)$. In practice, large language models (e.g., GPT) can serve as $\mathcal{S}$ to generate summarized text that forms a higher-level chunk. For example, a paragraph-level chunk $c_5$ may be obtained by compressing four consecutive sentence-level chunks $c_5 = \mathcal{S}(c_1, c_2, \dots, c_4)$. While raw fine-grained chunks preserve full semantic fidelity, they may fragment higher-level structure. Conversely, compressed chunks capture compact semantic summaries but may lose fine-grained details. This design enables the system to balance accuracy versus efficiency by adaptively mixing raw and compressed representations. \xz{didn't use $s$}

\textbf{Planner} The planner, denoted by $\mathcal{P}$, is a model that predicts the appropriate chunking granularity for a given query. Formally, $\mathcal{P}(q,MetaData(D)) = \left(\text{level}_{\min}, \; \text{level}_{\max}\right)$, where $\text{level}_{\min}, \text{level}_{\max}$ denote the smallest and largest chunk levels sufficient to answer $q$ while minimizing overall cost (including multi-level chunk construction, retrieval, and generation), $MetaData(D)$ denote the metadata of documents. These predictions restrict the candidate retrieval set to: $C = \{ c \in \mathcal{H}(D) \;|\; \text{level}(c) \in [\text{level}_{\min}, \text{level}_{\max}] \}$.

\textbf{Chunk Compression Encoder}
Beyond text-level summarization, we introduce an embedding-level compression module, denoted as $\mathcal{E}(\cdot)$. Unlike $\mathcal{S}(\cdot)$, which produces summarized text chunks, $\mathcal{E}(\cdot)$ directly maps a set of fine-grained chunks into a single compressed embedding without generating intermediate text. Formally, given a group of lower-level chunks $\{c_1, c_2, \dots, c_4\}$ the module outputs : $e(c_5) = \mathcal{E}(c_1, c_2, \dots, c_4) \in \mathbb{R}^d$. where $e(c_5)$ represents a high-level semantic embedding that captures the aggregate meaning of the input chunks. In practice, $\mathcal{E}$ can be a pretrained embedding model such as SBERT encoder (multi-qa-mpnet-base-cos-v1)~\cite{reimers-gurevych-2019-sentence}, long-context embedding model (jina-embeddings-v3)~\cite{sturua2024jina} or a finetuned Chunk Compression Encoder.
% \textbf{Retriever}
% As in a standard RAG pipeline, given the candidate set $C$, retrieval is performed by ranking chunks based on similarity between query embedding $e(q)\in \mathbb{R}^d$ and chunk embeddings $e(c)\in \mathbb{R}^d$. The top-$k$ chunks form:
% $
% \mathcal{R}(q, C) = \operatorname{TopK}\Big( \{ \langle e(q), e(c) \rangle : c \in C\} \Big),
% $. This formulation is agnostic to the underlying retrieval method. Any advanced retriever can be incorporated in place of simple similarity search.
\begin{figure}[h!]
\centering
% \vspace{-35pt}
\includegraphics[width=\textwidth]{stitch.pdf}
% \vspace{-15pt}
\caption{\small{Overview of the STITCH framework.}}%\vspace{-15pt}
\label{fig:algo}
% \end{wrapfigure}
% \vspace{-15pt}
\end{figure}

\subsection{Planner: Trained with synthetic data pipeline + STITCH }

The planner must satisfy several requirements to be effective in retrieval-augmented QA. Accuracy is essential, as errors in selecting chunk levels directly propagate to retrieval and degrade downstream answer quality. The planner should also operate under low latency, with a target reasoning length of fewer than 128 tokens (roughly one second on commodity hardware), ensuring practical deployment in interactive settings. Finally, the planner must exhibit adaptability, performing robustly across diverse domains, query types, and document structures. To address the challenges of training a planner, including unavailable ground-truth, noisy pseudo-labels, costly data collection, and unstable multi-objective optimization, we propose STITCH (\textbf{S}olve with RL, \textbf{T}hen \textbf{I}mitate \textbf{T}o \textbf{C}lose \textbf{H}oles), a robust and sample-efficient training framework. As illustrated in \Cref{fig:algo} and \Cref{alg:stitch_general}, STITCH combines reinforcement learning (RL) and supervised fine-tuning (SFT) in a stable loop:

% \begin{algorithm}[H]
% \caption{STITCH: Solve with RL, Then Imitate To Close Holes} \label{alg:stitch_general}
% \begin{algorithmic}[1]
% \Require Dataset $\mathcal{D}$, planner policy $\mathcal{P}_\theta$, batch size $N$, GRPO optimizer, Imitation learning(IL) buffer size $T$
% \State Initialize $B_{\text{IL}} \leftarrow \emptyset$
% \For{each training step}
%     \State Sample batch $\{(q_j, D_j, a_j)\}_{j=1}^N \sim \mathcal{D}$
%     \State Initialize RL buffer $B_{\text{RL}} \leftarrow \emptyset$
%     \For{each $(q, D, a)$ in batch}
%         \State Extract metadata $m \leftarrow \textsc{MetaData}(D)$
%         \State Sample vanilla rollouts $\{o_i\}_{i=1}^G \sim \mathcal{P}_\theta(\cdot \mid q, m)$
%         \If{\textsc{IsSolvable}$(\{o_i\}, a)$}
%             \State Add $(q, m, \{o_i\})$ to $B_{\text{RL}}$
%             \State \textbf{continue}
%         \EndIf
%         \State Generate hint $\rho \leftarrow \textsc{GenHintTrace}(q, D, a)$
%         \State Sample hinted rollouts $\{o_i'\}_{i=1}^G \sim \mathcal{P}_\theta(\cdot \mid q+\rho, m)$
%         \If{\textsc{IsSolvable}$(\{o_i'\}, a)$}
%             \State Add $(q+\rho, m, \{o_i'\})$ to $B_{\text{RL}}$
%         \Else
%             \State Get pseudo-label $y \leftarrow \textsc{GetChunkLabel}(q, D, a)$
%             \State Generate reasoning trace $\tau \leftarrow \textsc{GenTrace}(q, D, y)$
%             \State Add $(q, D, a, \tau)$ to $B_{\text{IL}}$
%         \EndIf
%     \EndFor

%     \If{$B_{\text{RL}} \neq \emptyset$}
%         \State \textsc{UpdatePolicyGRPO}$(\pi_\theta, B_{\text{RL}})$
%     \EndIf

%     \If{$|\mathcal{B}_{\text{IL}}| \geq T$}
%         \State \textsc{ImitationLearningStep}$(\mathcal{B}_{\text{IL}})$
%         \State Clear $\mathcal{B}_{\text{IL}}$
%     \EndIf
% \EndFor
% \end{algorithmic}
% \end{algorithm}
\begin{algorithm}[H]
\caption{STITCH: Solve with RL, Then Imitate To Close Holes} \label{alg:stitch_general}
\begin{algorithmic}[1]
\Require Dataset $\mathcal{D}$, planner policy $\mathcal{P}_\theta$, batch size $N$, GRPO optimizer, imitation learning (IL) buffer size $T$
\State Initialize $B_{\text{IL}} \leftarrow \emptyset$
\For{each training step}
    \State Sample batch $\{(q_j, D_j, a_j)\}_{j=1}^N \sim \mathcal{D}$
    \State Initialize RL buffer $B_{\text{RL}} \leftarrow \emptyset$
    \For{each $(q, D, a)$ in batch}
        \State Extract metadata $m \leftarrow \textsc{MetaData}(D)$
        
        \State \textcolor{gray}{\# Step 1: Vanilla RL rollout \#}
        \State Sample vanilla rollouts $\{o_i\}_{i=1}^G \sim \mathcal{P}_\theta(\cdot \mid q, m)$
        \If{\textsc{IsSolvable}$(\{o_i\}, a)$}
            \State Add $(q, m, \{o_i\})$ to $B_{\text{RL}}$
            \State \textbf{continue}
        \EndIf
        % \Comment{\# Step 3: Hinted RL rollout \#}
        \State \textcolor{gray}{\# Expert trace generation \#}
        \State Get pseudo-label $y \leftarrow \textsc{GetChunkLabel}(q, D, a)$
        \State Generate reasoning trace $\tau \leftarrow \textsc{GenTrace}(q, D, y)$
        \State \textcolor{gray}{\# Step 2: Hinted RL rollout \#}
        \State Generate hint $\rho \leftarrow \textsc{ExtractHintTrace}(\tau)$
        \State Sample hinted rollouts $\{o_i'\}_{i=1}^G \sim \mathcal{P}_\theta(\cdot \mid q+\rho, m)$
        \If{\textsc{IsSolvable}$(\{o_i'\}, a)$}
            \State Add $(q+\rho, m, \{o_i'\})$ to $B_{\text{RL}}$
        \Else
            % % \State \textcolor{gray}{ Step 3: Expert trace generation \#}
            % \State Get pseudo-label $y \leftarrow \textsc{GetChunkLabel}(q, D, a)$
            % \State Generate reasoning trace $\tau \leftarrow \textsc{GenTrace}(q, D, y)$
            \State Add $(q, D, a, \tau)$ to $B_{\text{IL}}$
        \EndIf
    \EndFor

    \State \textcolor{gray}{\# Policy update via GRPO \#}
    \If{$B_{\text{RL}} \neq \emptyset$}
        \State \textsc{UpdatePolicyGRPO}$(\pi_\theta, B_{\text{RL}})$
    \EndIf

    \State \textcolor{gray}{\# Step 3: Imitation learning on unsolved cases \#}
    \If{$|B_{\text{IL}}| \geq T$}
        \State \textsc{ImitationLearningStep}$(B_{\text{IL}})$
        \State Clear $B_{\text{IL}}$
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

We will first describe the algorithm at a high level, and the key results that support its design.
In \alg, for each question $q$ paired with the documents $D$ and answer $a$, the workflow of \alg is shown in \Cref{fig:algo} and proceeds as follows:
\begin{enumerate}[nosep,leftmargin=*]
    \item \textbf{Vanilla RL rollout:} In Step 1, we optimize the planner using vanilla RL. Given a task $(q,D)$, the planner generates a group of $G$ rollouts $\{o_i\}_{i=1}^G = \mathcal{P}(q,MetaData(D))$, where each rollout predicts a chunking granularity plan based on the query and document metadata. 
    For each rollout, we extract the predicted chunk sizes $\left(\text{level}_{\min}, \; \text{level}_{\max}\right)$ and execute the corresponding retrieval-augmented QA. If any rollout leads to a correct answer and satisfies the planning latency constraint, we mark the case as solvable and use it for policy updates.
    \vspace{4pt}

    \item \textbf{Hinted RL rollout:} If the question remains unsolved, we enter Step 2 (Hinted RL rollout). We generate an expert trace that solves the question while satisfying all constraints, and extract a short hint from this trace. This hint is appended to the question $(q,\rho)$ and used to condition a new RL rollout. If the hinted rollout succeeds, the planner is updated accordingly. \vspace{4pt}  
    % We will first generate a expert trace that can solve the question and follows all the constraints(length). So the input become question appended with the hint from the expert trace $(q,\rho)$, we will generate rollouts again the new sampled output group $\{o_i^\prime\}_{i=1}^G$, resulting from the question appended with the hint from the expert trace within a pre-defined range $(q,\rho)$.\vspace{4pt}
    \item \textbf{Imitation learning:} However, for hard cases that remain unsolved even with hints, we move to Step 3 (imitation learning). These examples are stored and periodically used to fine-tune the model via supervised learning, using full expert traces and answers.
    
%     \item \textbf{Expert trace generation:} 
%     To supervise the planner, we design a reasoning trace generation pipeline that produces pseudo-labels and diverse training traces. The process proceeds in four stages:
% \begin{enumerate}[nosep,leftmargin=*]
%     \item \textbf{Hierarchy Construction.} We first construct the complete chunk hierarchy, with the smallest unit corresponding to a sentence and the largest corresponding to the full document.
%     \item \textbf{Initial Retrieval.} Given a query, we perform top-k retrieval and use the retrieved chunks to generate an answer with a backbone model.
%     \item \textbf{Pseudo-Label Assignment.}
%     If the generated answer is correct, we record the smallest and largest chunk levels among the retrieved chunks as a pseudo-label. We emphasize that these pseudo-labels are not guaranteed to be optimal. If the answer is incorrect, we expand retrieval with additional chunks to check whether the model can then recover the correct answer.

%     \item \textbf{Reasoning Trace Generation.} We use the collected pseudo-labels to generate reasoning traces. To improve trace diversity and reduce overfitting, we sample traces from multiple large language models, including Llama3~\cite{grattafiori2024llama}, GPT-4o~\cite{hurst2024gpt}, Qwen3~\cite{yang2025qwen3}, and DeepSeek-R1~\cite{guo2025deepseek}, covering parameter scales from 1.5B to 671B.
% \end{enumerate}

%     \item \textbf{Policy updates:} Optimize the policy via the following objective:
%     {\footnotesize
%     \begin{align}
%         \mathcal{J}_{\text{STITCH}}&(\theta)=\mathbb{E}_{(q,\rho,a)\sim\mathcal{D},\{o_i\}_{i=1}^G\sim\pi_{\text{old}}(\cdot|(q,\rho))} \notag\\&\left[\frac{1}{G}\sum_{i=1}^G\frac{1}{|o_i|}\sum_{t=1}^{|o_i|}\left(\min\left(r_{i,t}(\theta)\hat{A}_{i,t},\text{clip}\left(r_{i,t}(\theta),1-\varepsilon,1+\varepsilon\right)\hat{A}_{i,t}\right)-\beta D_{\text{KL}}(\pi_\theta||\pi_{\text{ref}})\right)\right],
%     \label{eq:BREAD_obj}
%     \end{align}
%     }
%     where
%     {\footnotesize
%     \begin{align}
%         r_{i,t}(\theta)=\frac{\pi_{\theta}(o_{i,t}|q,\rho,o_{i<t})}{\pi_{\text{old}}(o_{i,t}|q,\rho,o_{i<t})},\quad \hat{A}_{i,t}=\frac{r_i-\text{mean}(\{R_i\}_{i=1}^G)}{\text{std}(\{R_i\}_{i=1}^G)}
%     \label{eq:adv}
%     \end{align}
%     }

\end{enumerate}
This training loop continues, alternating between RL and SFT, until convergence. STITCH enables stable learning under multi-objective reward, improves sample and computational efficiency, and produces a planner that generalizes across domains and document types with low latency.

\textbf{Policy updates:}
Solvable cases from either stage are used to update the policy with the following objective. The update balances reward, policy divergence, and planning efficiency:
    {\footnotesize
    \begin{align}
        \mathcal{J}_{\text{STITCH}}&(\theta)=\mathbb{E}_{(q,\rho,a)\sim\mathcal{D},\{o_i\}_{i=1}^G\sim\pi_{\text{old}}(\cdot|(q,\rho))} \notag\\&\left[\frac{1}{G}\sum_{i=1}^G\frac{1}{|o_i|}\sum_{t=1}^{|o_i|}\left(\min\left(r_{i,t}(\theta)\hat{A}_{i,t},\text{clip}\left(r_{i,t}(\theta),1-\varepsilon,1+\varepsilon\right)\hat{A}_{i,t}\right)-\beta D_{\text{KL}}(\pi_\theta||\pi_{\text{ref}})\right)\right],
    \label{eq:BREAD_obj}
    \end{align}
    }
    where
    {\footnotesize
    \begin{align}
        r_{i,t}(\theta)=\frac{\pi_{\theta}(o_{i,t}|q,\rho,o_{i<t})}{\pi_{\text{old}}(o_{i,t}|q,\rho,o_{i<t})},\quad \hat{A}_{i,t}=\frac{r_i-\text{mean}(\{R_i\}_{i=1}^G)}{\text{std}(\{R_i\}_{i=1}^G)}
    \label{eq:adv}
    \end{align}
    }

\textbf{RL Reward Components in STITCH}
To train the planner effectively, we design a multi-objective reward $R$ that balances several desiderata:
$$
R = R_{\text{QA}}  + R_{\text{Cost}} + R_{\text{Format}}+ R_{\text{Length}}
$$

Each term is defined as follows:
\begin{itemize}
\item QA Answer Correctness $R_{\text{QA}}$: 
$
R_{\text{QA}} = 
\begin{cases}
+1, & \text{if generated answer } a = a^{\text{gold}} \\
0, & \text{otherwise}
\end{cases}
$

\item Chunk Budget Penalty $R_{\text{Cost}}$: 
To encourage fewer, more informative chunks, we penalize the cost of building multi-level chunks $c$:
$
R_{\text{Cost}} = -\alpha \cdot \text{ChunkCost} 
$
\item  Trace Length Penalty $R_{\text{Length}}$: We penalize overly long traces beyond a target token budget $L_{\text{max}}$. Let $\ell$ be the number of generated tokens in the reasoning trace:
$
R_{\text{Length}} = -\beta \cdot \text{ReLU}(\ell - L_{\text{max}})
$
\item Format $R_{\text{Format}}$: To encourage structured reasoning and ensure the answer is extractable, we include a reward term that promotes outputs matching a predefined format. This is standard in reasoning-based models training.
$
R_{\text{Format}} = 
\begin{cases}
+\gamma, & \text{if matches format} \\
0, & \text{otherwise}
\end{cases}
$

 \item Pseudo-Label Alignment $R_{\text{PlanningAcc}}$: 
As an alternative to optimizing QA accuracy and efficiency tradeoff($R_{\text{QA}}  + R_{\text{Cost}}$), we introduce a reward that aligns the planner’s output with pseudo-labels. This bypasses retrieval and answer generation during training, enabling more stable and fast training. 

Specifically, if the predicted chunk bounds $(\hat{l}_{\min}, \hat{l}_{\max})$ match the pseudo-labeled bounds $(l_{\min}, l_{\max})$, we provide a positive reward:
$$
R_{\text{PlanningAcc}} = 
\begin{cases}
+1, & \text{if } \hat{l}_{\min} = l_{\min} \text{ and } \hat{l}_{\max} = l_{\max} \\
0, & \text{otherwise}
\end{cases}
$$
This term is particularly useful during early training to guide the model before it begins fully exploring the performance-efficiency trade-off on its own.

\end{itemize}
\textbf{Synthetic data pipeline}
To support this loop, we design a reasoning trace generation pipeline with four stages:
\begin{enumerate}[nosep,leftmargin=*]
    \item \textbf{Hierarchy Construction.} We first construct the complete chunk hierarchy, with the smallest unit corresponding to a sentence and the largest corresponding to the full document.
    \item \textbf{Initial Retrieval.} Given a query, we perform top-k retrieval and use the retrieved chunks to generate an answer with a backbone model.
    \item \textbf{Pseudo-Label Assignment.}
    If the generated answer is correct, we record the smallest and largest chunk levels among the retrieved chunks as a pseudo-label. We emphasize that these pseudo-labels are not guaranteed to be optimal. If the answer is incorrect, we expand retrieval with additional chunks to check whether the model can then recover the correct answer.

    \item \textbf{Reasoning Trace Generation.} We use the collected pseudo-labels to generate reasoning traces. To improve trace diversity and reduce overfitting, we sample traces from multiple large language models, including Llama3~\cite{grattafiori2024llama}, GPT-4o~\cite{hurst2024gpt}, Qwen3~\cite{yang2025qwen3}, and DeepSeek-R1~\cite{guo2025deepseek}, covering parameter scales from 1.5B to 671B.
\end{enumerate}
This pipeline enables automatic construction of supervision signals that are both diverse and scalable, providing a foundation for robust planner training. We shown ablation experiments of sample traces from multiple large language models or a single LLM in \Cref{exp:trace_diverse}.

The details of the algorithm can be found in \Cref{alg:STITCH}.
Next, we will discuss the key observations that motivate the design of \alg.

\textbf{Design choices and justifications.}
We next discuss the key design choices of STITCH.

\textbf{\emph{(1) Planning as More Than Classification.}}
At first glance, predicting planning signals such as smallest or largest chunk sizes may seem like a straightforward classification problem. But simple classification ignores the structured and sequential nature of planning~\cite{london2016stability}, which involves balancing a trade-off between retrieval cost and answer quality. Unlike classification, a reasoning model can capture this ambiguity through explicit traces that encode conditional logic and deep thinking (e.g., factual queries favor finer chunks, while synthesis tasks require larger spans). Theoretical work in structured prediction demonstrates that introducing intermediate latent variables reduces sample complexity and improves generalization under non-linear mappings~\cite{bello2018learning,li2021towards}, suggesting that reasoning traces serve as scaffolding to stabilize learning and improve robustness to distribution shift. Our ablation experiments further confirm this: simple MLP routers or LLMs without reasoning underperform compared to a finetuned SLM, showing the necessity of explicit reasoning for planning. Most importantly, reasoning-based planners exhibit stronger transfer across tasks and domains, consistent with insights from compositional generalization~\citep{wei2022chain,NEURIPS2024_8f395480}.


\textbf{\emph{(2) Add hint to build curriculum learning}}
Reasoning problems are inherently compositional hence we need a chain-of-thought \citep{wei2022chain} to solve such problems. Suppose the problem contains $T$ steps/subtasks to solve, each with successful completion probability of $\eps$ for the base student model. Then, we receive a final trajectory-level correctness reward with probability of $\eps^T$ assuming steps are independently completed. In contrast, by branching out from the expert trace at step $T-\tau$, STITCH only needs to complete the $\tau$ downstream steps, increasing the success to $\eps^{\tau}$. Notably, by increasing $\tau$ from $1$ to $T$, STITCH facilitates curriculum learning by tackling individual problem steps one at a time requiring only $\Omega(1/\eps)$ samples to attain success per step. Below we further formalize this discussion under a Markov chain model. \xz{ablation} 

\textbf{\emph{(3) If a question is hard, start by memorizing}}
RL-based training relies on preference or correctness rewards, which can be sparse and unstable. In contrast, SFT provides a strong fallback: the student memorizes canonical traces, ensuring coherence and baseline ability even on hard questions. This aligns with cognitive intuition: humans first memorize worked examples before refining their skills through exploration. Thus, SFT is not merely an initialization step but an essential safeguard against RL instability.

\textbf{\emph{(4) Sample diverse trace to avoid SFT overfitting}}
A key risk of pure SFT is overfitting to a narrow distribution of traces, which can cause models to fail on semantically valid but stylistically different reasoning patterns. It is also known that an $L$-times deeper LLM can internally simulate $L$ chain-of-thought steps of a smaller LLM~\cite{saunshi2025reasoning}. Consequently, expert models often generate long and dense traces that are prohibitively difficult for small student models to digest in one stage of supervised fine-tuning (SFT). Without proper strategy, the student may fail to align with the expert. Recent work~\cite{li2025small} provides empirical evidence that small language models indeed struggle to learn directly from strong reasoners. To mitigate this, we deliberately sample traces from diverse expert models (e.g., LLaMA, GPT, Qwen, DeepSeek across scales). Theoretically, this expands the student’s support over reasoning space, reducing variance in downstream generalization error. Empirically, it ensures robustness to varied reasoning styles, thereby preventing over-specialization to a single teacher.
\subsection{compressor}

A straightforward approach to obtaining high-level chunk embeddings is to first generate a summary with a LLM and then encode that summary using an embedding model. Formally, given a group of fine-grained chunks $\{c_1, \dots, c_m\}$, we obtain a summarized text chunk via an LLM:
$
\hat{s} = \mathcal{S}(c_1, \dots, c_m),
$
and its embedding using a pretrained encoder $\epsilon$:
$
e_{\text{gt}}= \epsilon(\hat{s}) \in \mathbb{R}^d.
$
This provides a ground-truth compressed embedding $e_{\text{gt}}$. However, this pipeline is expensive because it requires repeated calls to the LLM $\mathcal{S}$.

To reduce cost, we train a lightweight compression model $\mathcal{S}$ that maps a set of lower-level chunk embeddings directly into a high-level compressed embedding:
$
e_{\text{comp}} = \mathcal{S} \big( \epsilon(c_1), \dots, \epsilon(c_m) \big).
$
The compression model is trained to minimize the discrepancy between its output $e_{\text{comp}}$ and the ground-truth embedding $e_{\text{gt}}$:
$
\mathcal{L}_{\text{comp}}(\mathcal{S}) = \big\| e_{\text{comp}} - e_{\text{gt}} \big\|_2^2.
$
Once trained, $\mathcal{S}$ can directly produce high-level embeddings without requiring LLM summarization, yielding comparable retrieval accuracy at much lower cost in both compute and latency.

\textbf{Design choices and justifications.} We next discuss the key design choices.

\textbf{\emph{(1) Why we need summarization.}}
Transformer-based encoders (e.g., SBERT \cite{reimers-gurevych-2019-sentence}, E5 \cite{wang2022text}) degrade when applied to very long spans. Summarization condenses essential semantics into a shorter sequence before encoding, yielding embeddings that better capture document-level meaning. Works like RAPTOR \cite{sarthi2024raptor} and MALRAG \cite{zheng2025multiple} show that hierarchical RAG benefits from summarized nodes: summaries act as “semantic bottlenecks,” discarding redundancy while keeping high-level signals. Without summarization, embeddings of concatenated raw text tend to overweight surface-level lexical overlap rather than conceptual structure. Recent retrieval benchmarks (e.g., \cite{kamradt2024levels, asai2024self}) report that embeddings of summaries achieve higher recall and downstream QA accuracy than embeddings of raw large chunks, especially for multi-hop queries requiring abstraction. \xz{see ablation}

\textbf{\emph{(2) Summarization changes the representation.}}
Summarization alters the text distribution, which in turn changes its embedding representation. As a result, embeddings of summaries are not equivalent to embeddings of the original content, motivating the need for a dedicated compression model. \xz{see ablation}

